Exploring Universal Intrinsic Task Subspace via Prompt Tuning

Why can pre-trained language models (PLMs) learn universal representations and effectively adapt to broad NLP tasks differing a lot superficially? In this work, we empirically find evidence indicating that the adaptations of PLMs to various few-shot tasks can be reparameterized as optimizing only a few free parameters in a unified low-dimensional intrinsic task subspace, which may help us understand why PLMs could easily adapt to various NLP tasks with small-scale data. To find such a subspace and examine its universality, we propose an analysis pipeline called intrinsic prompt tuning (IPT). Specifically, we resort to the recent success of prompt tuning and decompose the soft prompts of multiple NLP tasks into the same low-dimensional nonlinear subspace, then we learn to adapt the PLM to unseen data or tasks by only tuning parameters in this subspace. In the experiments, we study diverse few-shot NLP tasks and surprisingly find that in a 250-dimensional subspace found with 100 tasks, by only tuning 250 free parameters, we can recover 97% and 83% of the full prompt tuning performance for 100 seen tasks (using different training data) and 20 unseen tasks, respectively, showing great generalization ability of the found intrinsic task subspace. Besides being an analysis tool, IPT could further help us improve the prompt tuning stability.

==> sections/6_discussions.tex <==
\section{Discussion}
\paragraph{Could NLP tasks be reparameterized into the same subspace?}
We find strong evidence for this hypothesis with our \ourmodel pipeline, which can find subspaces containing sub-optimal but non-trivial solutions for PLM adaptations to unseen data and tasks. However, the achieved performance of \ourmodel is still far from perfect, and increasing $d_I$ does not significantly improve it. Although it may come from the inadequacy of current subspace-finding methods and optimization algorithms, based on current results, we cannot directly conclude that PLM adaptations to various NLP tasks could be reparameterized into exactly the same subspace. However, at least we have found promising empirical results showing that the low-dimensional reparameterization subspaces of various tasks have a substantial \textbf{intersection}, which MSF is designed to find. We thus encourage future work to explore (1) how to improve \ourmodel to find stronger evidences, and (2) whether the \textbf{union} of reparameterization subspaces for various tasks is also low-dimensional.

% , since the MSF's training objective is essentially to find the intersections for the compressed objective landscapes by jointly optimizing all the task-specific objectives and it works for compressing training tasks and can also generalize to unseen tasks to some extent. Supposing the compressed low-dimensional subspaces randomly distribute in the very-high-dimensional full parameter space, it should be almost impossible for them to have a substantial intersection. We encourage the future work to explore whether the union of low-dimensional subspaces compressing various tasks is also low-dimensional.

%Moreover, it shoud also be noted that the extremely low dimension (about $5\sim100$) achieved by \ourmodel should not be regarded exactly as \textit{intrinsic dimension} of~\cite{aghajanyan-etal-2021-intrinsic} and~\cite{li2018measuring} since the \textit{intrinsic dimension} should ensure that the satisfying performance can be achieved in that low dimension. The dimension achieved with \ourmodel could roughly serve as a lower bound for the \textit{intrinsic dimension}.

% \paragraph{Measuring Task Differences with \ourmodel.}

\paragraph{Relation to the scaling law.}
Recently, people have found that larger PLMs tend to be more sample-efficient~\citep{Kaplan2020ScalingLF}, parameter-efficient~\citep{lester2021power} and cross-task generalizable~\citep{Wei2021FLAN}. Our research hypothesis may help to understand this phenomenon: the adaptations of larger PLMs can be better reparameterized into a unified subspace so that the cross-task generalization will be easier, and larger PLMs have lower reparameterization dimensions~\citep{aghajanyan-etal-2021-intrinsic}, hence they should need less data and tunable parameters. This also implies that the characteristics of intrinsic task subspaces may be used to examine whether a PLM is well trained. 

%If this hypothesis holds, we argue that tuning methods similar to \ourmodel should be developed. Larger PLMs provide much stronger compression framework and we can find the low-dimensional intrinsic task subspaces and train various downstream tasks in these subspaces, which will avoid the instability and large generalization gap caused by over-parameterization and also be greener to environments.

\paragraph{Utilize and manipulate intrinsic vectors.} The intrinsic vectors obtained during IST depict the adaptations to different tasks and it is worthwhile to explore whether we can (1) utilize them to find the relationships between different tasks, and (2) manipulate these vectors to achieve some interesting cross-task generalization results.

\paragraph{Tuning PLMs within intrinsic task subspaces.}
We have demonstrated in Table~\ref{tab:variance} and \cref{sec:combine} that \ourmodel  can improve tuning stability. We encourage to explore more methods to tune PLMs within low-dimensional intrinsic task subspaces, which may have more practical benefits such as avoiding over-parameterization and being greener to environments with less tuneable parameters.

% \paragraph{Atomic Operation for NLP tasks.}
